Sponsored Question Answering

The potential move from search to question answering (QA) ignited the question of how should the move from sponsored search to sponsored QA look like. We present the first formal analysis of a sponsored QA platform. The platform fuses an organic answer to a question with an ad to produce a so called {\em sponsored answer}. Advertisers then bid on their sponsored answers. Inspired by Generalized Second Price Auctions (GSPs), the QA platform selects the winning advertiser, sets the payment she pays, and shows the user the sponsored answer. We prove an array of results. For example, advertisers are incentivized to be truthful in their bids; i.e., set them to their true value of the sponsored answer. The resultant setting is stable with properties of VCG auctions.

==> log.tex <==
\subsection{Sponsored content generation}

In the defined setup, the whole game is conducted with predetermined sponsored contents of the advertisers. We propose a possible process through which these sponsored contents are generated. In this section, we develop a formalism of a generation process induces the distribution of sponsored contents for every advertiser. In the next section we demonstrate an example of a unigram generation process and analyze it in through our proposed framework. \\

Let assume an LLM-based QA platform is asked a question $q \in \textk$ and wish to generate an answer with an ad $d \in V^{k}$ integrated in it. As described in \cite{feizi_online_2024}, we assume the platform is responsible for generating the sponsored content, and not the advertiser itself.
***Oren***:we shifted back to question from query in the begining of section 5.
***Tommy***: fixed.
**** Moshe: Assume "their approach" in the paragraph above (phrasing ??) and below "propose approaches" need some re-phrasing ****
****Tommy: i repharse a bit and foucus on cases the generated sponsored content is a distribution over all string of k tokens****

% \textbf{The first} approach is a lexical representation of the generated sponsored content, i.e the output of the generation process is a series of tokens.
% \textbf{The second} approach is a language model (LM) representation of the generated sponsored content, i.e the output of the generation process is a language model (LM).

*****Moshe: I think it is unclear what it means the output is LM; at some point it should be format what is an inoy and what is the output in formal terms in both cases ****
***Tommy: done***
***Oren***: coming to think about it, is it really sampled? you have d and you mix it with an ad; both are texts (which were already drawn from a distribution). Unless we are going to sample from the distributions that generated them. I will wait to see.
***Tommy***: i fix everything, so it will be clear start the game  with a fixed $d^{*}$, not matter how they were generated.

We suggest the sponsored content is sampled from a distribution induced from a generation process. Conceptually, the process of generating a sponsored content, may be composed from two sub generators: the first generator aims to satisfy the user's information need, i.e answer the asked question. The second generator aims to incentive the advertiser, i.e increase the alignment of the generated sponsored content to the advertiser's advertisement.
In order to combine both generators in a unite process of generating sponsored content, we define a one dimensional mixture parameter, that controls the balance between those two generators. A formal definition:\\
\begin{definition} 
A \textit{Generation} of sponsored content given a question $q \in V^{k}$, an ad $d \in V^{k}$  and a mixture parameter $\lambda \in [0,1]$ is defined as the function:
    % \item For the first approach of representing sponsored content: $g:V^{\leq k} \times V^{\leq k} \times [0,1] \xrightarrow[]{} V^{\leq k}$ where $V^{\leq k}, V^{\leq k}$ are documents of maximum length of $k, k$, respectively.
% For the second approach of representing sponsored content: 
$g:\textk \times \textk \times [0,1] \xrightarrow[]{} \distk$  where $\distk$ is a set of all distributions over the set of all series of tokens with length of $k$.
We sign an \textbf{instance} of a sponsored content as $d^{SC}\sim g(q, d, \lambda)$. XXX
***Oren***: again we shift to a query.
***Tommy***: fixed to question.
***Oren***:no need to remention given that it was already stated.
***Tommy***: deleted.
\end{definition}
% Note that the generation process can be design as any stochastic process, s.t auto-regressive, markov-process, etc 
% *** [Oren,Moshe - should we give some examples here?]. \\

***Oren***: An LLM based example can help where the LLM is asked to merge q and d with some weight lambda and accordingly generates a distribution (albeit other single tokens but this can be extended to sequences).
***Tommy***: i omit this for now.

The mixture parameter $\lambda$ control the balance between the generator of the pure answer $\pure$ to question $q$ and the generator of the advertiser $d$. W.l.o.g we assume when $\lambda$ increase (approaching 1), the sponsored content becomes more aligned with the pure answer (and less influenced by the advertisement). Conversely, As $\lambda$ decrease (approaching 0), the sponsored content becomes more aligned with the advertisement and less focused on the pure answer.
***Oren***: there is a subtle point here; say that g uses the mixture of the LMs generated q and d; so the resultant mixture is a distribution; lambda doesn't really give more weight to q or d but rather to the generator from which they were generated.
***Tommy***: i am not sure i get your point. lambda define to which generator give more weight, and that controls the balance between answering to $q$ and generating tokens from the advertisement.

***** Moshe: notice that if we use a probabilistic procedure then $d^{SC}$ is a random variable, so we should later on might need to treat at such. For example, if you decide on your bid before $g$ is applied you can only know your expected value while determining the bid. In general we should be careful with what are given, what is generated, and whether these are strings, random strings, etc.  *****  
*** Tommy: We talked today that for now we use a specific serie of k tokens of the sponsored content, sampled from the stochastic generation process. (a specific series is given an advertiser to bid on).  The similarities are calculated over those probability distributions as well .  ***

 **** Moshe: In the above definition: when do we specify how the mixture works? How exactly weights are given? In the second approach: do we have generate token by token, while generating prefix? These should be crystalllized.  ****
 ***Tommy: I hope now its better***



 As a demonstration of the framework of sponsored content game and a generation process of sponsored contents, we present a 2-advertisers game with a unigram language model used both to generate the sponsored contents and to represent texts while calculating their similarities, as usually done in information retrieval systems\cite{raiber_kullback-leibler_2017}. We begin with a definition of a unigram generation process that induce a distribution from which we sample sponsored contents and discuss several similarity metrics of texts represented by a unigram model, based on commonly known distance metrics. Moreover, we present two properties of the mechanism, reflected in the unigram case.

 We suggest several valid similarity metrics of unigram language models.
\subsubsection{Shifted Negative Jensen–Shannon divergence}
We remind the Jensen–Shannon divergence (JSD) of $Z, Q \in \Delta(V)$ is defined as $JSD(Z||Q) = \frac{1}{2}D_{KL}(Z||M) + \frac{1}{2}D_{KL}(Q||M)$ where $M = \frac{1}{2}(Z+Q)$. JSD has several useful properties.: (1) JSD is symmetric in $Z, Q$; (2) JSD is bounded: $0 \leq JSD(Z||Q)\leq 1$; and (3) JSD is convex. In order to get a valid similarity metric, we define a shifted negative version of JSD as: $\forall d_a, d_b \in \Delta(V): S(d_a, d_b) = 1 - JSD(d_a || d_b)$ \footnote{We abuse the notation of JSD and write $JSD(d_a||d_b)$ instead of $JSD(p(t|d_a)||p(t|d_b))$}.
\subsubsection{Shifted Negative Cross Entropy}
We reformulate the Cross Entropy function to obtain a valid similarity metric. Let define a Shifted negative Cross Entropy (CE) as $\forall d_a, d_b: S(d_a, d_b) =
A - CE(d_a||d_b)$. where $A = max_{j_1, j_2}(\{CE(d_{j_1}||d_{j_2}) | d_{j_1}, d_{j_2} \in {d_0} \cup \{d_i\}_{i\in N}\})$\footnote{We abuse the notation of CE and write $CE(d_a||d_b)$ instead of $CE(p(t|d_a)||p(t|d_b))$}.
Let derive the Social Welfare of showing document $d^{SC}_{i}$ and use the linear dependency in the first argument of CE: \\
$SW(d^{SC}_{i}, d_i, d_0) = S(d^{SC}_{i}, d_0) + S(d^{SC}_{i}, d_i) = A - CE(d^{SC}_{i}||d_0) + A - CE(d^{SC}_{i}||d_i) = 2 \cdot A - (\lambda_i CE(d_0||d_0) + (1-\lambda_i) CE(d_i||d_0)) - (\lambda_i CE(d_0||d_i) + (1 - \lambda_i) CE(d_i||d_i)) = 2 \cdot A - CE(d_i||d_0) - CE(d_i||d_i) + \lambda_i (CE(d_i||d_0) + CE(d_i||d_i) - CE(d_0||d_0) - CE(d_0||d_i))$. \\
We suggest a symmetric version of this similarity metric:

